Learning An Active Inference Model of Driver Perception and Control: Application to Vehicle Car-Following

In this paper we introduce a general estimation methodology for learning a model of human perception and control in a sensorimotor control task based upon a finite set of demonstrations. The model's structure consists of i the agent's internal representation of how the environment and associated observations evolve as a result of control actions and ii the agent's preferences over observable outcomes. We consider a model's structure specification consistent with active inference, a theory of human perception and behavior from cognitive science. According to active inference, the agent acts upon the world so as to minimize surprise defined as a measure of the extent to which an agent's current sensory observations differ from its preferred sensory observations. We propose a bi-level optimization approach to estimation which relies on a structural assumption on prior distributions that parameterize the statistical accuracy of the human agent's model of the environment. To illustrate the proposed methodology, we present the estimation of a model for car-following behavior based upon a naturalistic dataset. Overall, the results indicate that learning active inference models of human perception and control from data is a promising alternative to black-box models of driving.

==> macro.tex <==
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsthm}

\usepackage{graphicx}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{epstopdf}
% \usepackage{subfigure}
\usepackage{color}
\usepackage{multirow}
 
\usepackage{verbatim}
%\usepackage{galois}
\usepackage{algorithm,algorithmicx,algpseudocode}
%\usepackage[titletoc]{appendix}
\usepackage{cite}
\usepackage{bbm}
\usepackage{bigstrut}
%\usepackage[left=1in,top=1in,right=1in,bottom=1in,letterpaper]{geometry}
\usepackage[linktocpage,colorlinks,linkcolor=blue,anchorcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{cleveref}

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
%\providecommand{\keywords}[1]
%{\small	
%  \textbf{\textit{Keywords---}} #1
%}

%\newcommand{\setword}[2]{%
%	\phantomsection
%	#1\def\@currentlabel{\unexpanded{#1}}\label{#2}%
%}
%\makeatother
\newcommand{\bl}{\color{blue}}
\newcommand{\rd}{\color{red}}


\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother



\usepackage{textcase}
\usepackage[tablename=TABLE]{caption}
\DeclareCaptionTextFormat{up}{\MakeTextUppercase{#1}}
\captionsetup[table]{
	labelsep=period,
	justification=centering,
	textformat=up,
}
%\usepackage[font=sc]{caption}
%\makesavenoteenv{tabular}
%\makesavenoteenv{table}
\numberwithin{equation}{section}
\crefname{equation}{equation}{equations}
\crefname{section}{Section}{Sections}

\newtheorem{theorem}{Theorem}%[section]
\crefname{theorem}{Theorem}{Theorems}
\crefname{definition}{Definition}{Definitions}

\newtheorem{corollary}{Corollary}%[theorem]
\newtheorem{lemma}{Lemma}%[theorem]
\crefname{lemma}{Lemma}{Lemmas}

\newtheorem{proposition}{Proposition}%[theorem]
\crefname{proposition}{Proposition}{Propositions}

\newtheorem{definition}{Definition}%[theorem]
\newtheorem{fact}{Fact}%[theorem]
\crefname{fact}{Fact}{Facts}
\crefname{corollary}{Corollary}{Corollaries}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}%[section]
\crefname{assumption}{Assumption}{Assumptions}
\crefname{algorithm}{Algorithm}{Algorithms}

\newtheorem{remark}{Remark}
\crefname{remark}{Remark}{Remark}
\newtheorem{question}{Question}[section]


\newcommand{\A}{\mathcal{A}}
 
\newcommand{\G}{\mathcal{G}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\cT}{\mathcal{T}} 
\newcommand{\cL}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
 



\newcommand{\cM}{\mathcal{M}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cX}{\mathcal{X}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bF}{\mathbf{F}}
%\newcommand{\ba}{\mathbf{a}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}


\newcommand{\bbI}{\mathbb{I}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\etal}{ et al. }
\newcommand{\br}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
%\newcommand{\Proj}{{\rm Proj}}
\newcommand{\half}{\frac{1}{2}}

\newcommand{\X}{\mathbf{x}}
\newcommand{\Y}{\mathbf{y}}
\newcommand{\Z}{\mathbf{z}}
\newcommand{\one}{\mathbf{1}}

% \newcommand{\bx}{\mathbf{x}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bad}{\begin{aligned}}
\newcommand{\ead}{\end{aligned}}
%\renewcommand{\arraystretch}{0.8}%
\newcommand{\normone}[1]{\| #1 \|_1}
\newcommand{\normtwo}[1]{\| #1 \|_2}
\newcommand{\abs}[1]{| #1 |}
\newcommand{\norminf}[1]{\| #1 \|_{\infty}}
\newcommand{\normfro}[1]{\| #1 \|_{\text{F}}}
\newcommand{\normfroinf}[1]{\| #1 \|_{\text{F},\infty}}
\newcommand{\normtwoinf}[1]{\| #1 \|_{2,\infty}}
\newcommand{\normop}[1]{\| #1 \|_{op}}

\newcommand{\inp}[2]{\left\langle #1, #2 \right\rangle}
%\newcommand{\setword}[2]{\phantomsection #1\def\@currentlabel{\unexpanded{#1}}\label{#2}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}

\newcommand{\lineSearch}{\mathop{\rm line\_search}}
\newcommand{\Line}{\mathop{\rm Line}}

 
\newcommand{\p}{\mathcal{P}}
\newcommand{\ps}{\mathcal{P_{\St}}}
\newcommand{\pt}{\mathcal{P_{\T}}}

\newcommand{\psm}{\mathbf{Proj_{\St}}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\disttwo}{ {d}_2}
\newcommand{\distinfty}{ {d}_{2,\infty}}


\newcommand{\sym}{\mathrm{sym}}
\newcommand{\Retr}{\mathrm{Retr}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\GG}{\mathrm{G}}
\newcommand{\T}{\mathrm{T}}
 \newcommand{\Prox}{{\rm Prox}}
\newcommand{\st}{\mathrm{s.t. }}
\newcommand{\ie}{\mathrm{i.e. }}
\newcommand{\vet}{\mathrm{vec}}
\newcommand{\St}{\mathrm{St}}
\newcommand{\TV}{\mathrm{TV}}
 \newcommand{\grad}{\mathrm{grad}}
 \newcommand{\Hess}{\mathrm{Hess}}
\newcommand{\vvec}{\mathrm{vec}}
\newcommand{\svec}{\overline{\mathrm{vec}}}
%\newcommand{\svec}{\textrm{svec}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\Proj}{\mathrm{Proj}}
%\def\red#1{\textcolor{red}{#1}}
%\def\blue#1{\textcolor{blue}{#1}}
\newcommand{\Exp}{\mathrm{Exp}}
\newcommand{\Log}{\mathrm{Log}}

\newcommand{\blue}{\color{blue}}
\newcommand{\red}{\color{red}}



\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note: } #1]}}
